Flatland Competition 2020: MAPF and MARL for Efficient Train Coordination on a Grid World

The Flatland competition aimed at finding novel approaches to solve the vehicle re-scheduling problem (VRSP). The VRSP is concerned with scheduling trips in traffic networks and the re-scheduling of vehicles when disruptions occur, for example the breakdown of a vehicle. While solving the VRSP in various settings has been an active area in operations research (OR) for decades, the ever-growing complexity of modern railway networks makes dynamic real-time scheduling of traffic virtually impossible. Recently, multi-agent reinforcement learning (MARL) has successfully tackled challenging tasks where many agents need to be coordinated, such as multiplayer video games. However, the coordination of hundreds of agents in a real-life setting like a railway network remains challenging and the Flatland environment used for the competition models these real-world properties in a simplified manner. Submissions had to bring as many trains (agents) to their target stations in as little time as possible. While the best submissions were in the OR category, participants found many promising MARL approaches. Using both centralized and decentralized learning based approaches, top submissions used graph representations of the environment to construct tree-based observations. Further, different coordination mechanisms were implemented, such as communication and prioritization between agents. This paper presents the competition setup, four outstanding solutions to the competition, and a cross-comparison between them.

==> Flatland Competition NeurIPS 2020/teams/an_old_driver.tex <==

\subsection{Multi-Agent Path Finding for Large-Scale Rail Planning}

Team \textit{An\_Old\_Driver}: Jiaoyang Li, Zhe Chen, Yi Zheng, Shao-Hung Chan; 1st place OR and overall.

% Jiaoyang Li, University of Southern California, jiaoyanl@usc.edu \\
% Zhe Chen, Monash University, zhe.chen@monash.edu \\
% Yi Zheng, University of Southern California, yzheng63@usc.edu \\
% Shao-Hung Chan, University of Southern California, shaohung@usc.edu \\


\subsubsection{Method}
The Flatland Challenge at its core is a MAPF problem. The first two differences discussed in \sectionref{sec:methods} can be addressed by small modifications of existing MAPF algorithms. The last difference, namely the malfunctions, can be handled during execution~\citep{MaAAAI17}. We therefore first plan collision-free paths under the assumption that no malfunctions occur in the beginning and then handle malfunctions once they occur.

\paragraph{Planning Collision-Free Paths}
We use Prioritized Planning (PP)~\citep{WHCA}, a simple but widely-used MAPF algorithm to generate the initial collision-free paths for all trains.
PP first sorts all trains in a priority ordering and then, from the highest priority to the lowest priority, plans a shortest path for each train while avoiding collisions with the already planned paths of higher-priority trains.
For efficiency, we use \emph{Safe Interval Path Planing} (SIPP)~\citep{SIPP} instead of A* to plan each such path in PP, since it avoids temporal symmetries. 

Although PP can find collision-free paths rapidly, its solution quality is far from optimal.
We therefore use Large Neighborhood Search (LNS)~\citep{LNS} to improve the solution quality. 
We follow \citet{LiAAMAS21} by using PP to generate an initial solution and repeating a neighborhood search process to improve the solution quality until the iteration limit is reached. In each iteration, we select a subset of trains and replan their paths using PP. The new paths need to avoid collisions with each other and with the paths of other trains. We adopt the new paths if they result in a smaller sum of the travel times.
As the Flatland Challenge provides 4 CPUs for evaluation, we run 4 LNS in parallel in practice. As we are given an overall runtime limit of 8 hours, we use simulated annealing to decide the iteration limit for each environment.

Although SIPP runs significantly faster than A*, it is still slow when there are thousands of trains because, as the paths of more trains are planned, SIPP has to plan paths that avoid collisions with more existing paths, resulting in its runtime growing rapidly.
We therefore propose a \emph{lazy planning} scheme where we plan paths only for some of the trains in the beginning, then let the trains move, and plan paths for the rest of trains during execution. 
Although delaying the planning time of the trains may delay their departure times, which in turn may delay their arrival times, lazy planning has two implicit benefits: (1) it avoids pushing too many trains to the environment at once, which could potentially prevent severe traffic congestion; and (2) when planning paths during execution, we take into account the influence of the malfunctions that have already happened or are happening.



\paragraph{Recovering from Malfunctions}

When a train encounters a malfunction during execution, deadlocks could happen if the trains stick to their original paths.
\emph{Minimum Communication Policies} (MCP)~\citep{MaAAAI17} avoids the deadlocks by stopping some trains to maintain the ordering that each train visits each location. It guarantees that all trains can reach their target stations within a finite number of timesteps. 
However, MCP sometimes may stop trains unnecessarily. We therefore develop a \emph{partial replanning} mechanism to avoid such unnecessary waits. When train A encounters a malfunction at some timestep, we collect all switch and crossing rail segments that train A is going to visit in the future and then collect the trains who are going to visit at least one of these rail segments after train A. We replan the paths of these trains in the prioritized planning manner and terminate when either new paths are planned for all of these trains or the runtime limit is reached.

\subsubsection{Results}

Our solution is implemented in C++ and is available from our public repository.\footnote{\url{https://github.com/Jiaoyang-Li/Flatland}} Our basic solution, namely PP with A* (instead of SIPP) plus MCP, solved 349 instances within 8 hours with a score of 282.56. When we replace A* with SIPP, our solution solved 3 more instances with a score of 285.4. LNS then improved the score to 289.1, and partial replanning further improved it to 291.873. Eventually, with the help of lazy planning, we solved 362 instances and reached our highest score of 297.5.
More details can be found in \citep{LiICAPS21}.


==> Flatland Competition NeurIPS 2020/teams/jbr_hse.tex <==
\subsection{PPO with Communication and Departure Schedule}
\label{sec:rl1}

Team \textit{JBR\_HSE}: Konstantin Makhnev, Oleg Svidchenko, Vladimir Egorov, Dmitry Ivanov, Aleksei Shpilman; 1st place RL.

% Konstantin Makhnev, HSE University, mah.kons@gmail.com\\ 
% Oleg Svidchenko, JetBrains Research and HSE University, oleg.svidchenko@jetbrains.com\\ 
% Vladimir Egorov, JetBrains Research and HSE University, vladimirrim98@gmail.com \\ 
% Dmitry Ivanov, JetBrains Research and HSE University, diivanov@hse.ru\\ 
% Aleksei Shpilman, JetBrains Research and HSE University, alexey@shpilman.com


\subsubsection{Method}

Our solution is based on Proximal Policy Optimization (PPO) \citep{PPO} enhanced with between-agent communication.
Communication has been shown to help agents to solve simple coordination problems \citep{CommNet,TarMAC}, and our solution extends this result to the complex Flatland environment.

\paragraph{Rewards} 

For each agent, its reward is defined as $0.01 \times \Delta d - 5 \times \texttt{is\_deadlocked} + 10 \times \texttt{has\_finished}$, where $\Delta d$ is the difference between the minimal distances to the destination point from its previous and current positions, and \texttt{is\_deadlocked} and \texttt{has\_finished} are the respective indicators of whether the agent is deadlocked or has successfully completed the episode.


\paragraph{Architecture}

In our solution, the agents are based on the actor-critic framework.
The actor makes decisions whenever encountering a switch, based on features from three sources (see \figureref{fig:architecture} in \appendixref{app:architecture}):

First, it receives information about the agent itself, such as its position on the map and indicators of whether it is deadlocked or malfunctioning. At the beginning of the episode, each agent is also assigned with a handle, a random number uniformly sampled from $[0, 1]$ which is supposed to represent priority. This information is processed with a fully-connected network (denoted as ``Common Features Net'').

Second, the actor observes the most relevant part of the map, encoded as the edges of a tree with a depth limited to 3. The features of each edge include its length, distance to the destination from its nodes, as well as information about other agents, including their positions and handles. The features of different edges are combined with a recursive network (denoted as ``Tree Features Net''), albeit replacing it with a fully-connected network produces similar performance.

Third, prior to action selection, the actor receives a set of floating-point vector messages generated by the neighbouring agents, i.e. the agents observed on the tree. Similarly to ATOC \citep{ATOC}, the messages are processed with self-attention layers \citep{attention}.

All components are trained end-to-end using PPO. The agents share experiences and network parameters. The architecture of the critic is similar to that of the actor, except the critic does not condition on communication signals. For a more complete description of the architecture and the features, please refer to our code.\footnote{\url{https://github.com/jbr-ai-labs/NeurIPS2020-Flatland-Competition-Solution}}


\paragraph{Departure Schedule}

To limit the maximum occupancy, we introduce a departure schedule. After pre-training agents without the schedule, we train a supervised classifier that determines the chances that each agent reaches its destination. Then, we only allow each train to start moving if the predicted probability exceeds a threshold, set to 0.92 at the start of the episode, and gradually lowered over time.


\subsubsection{Results}

We found that a carefully tuned PPO with simple heuristics for launching agents can achieve results comparable to simple algorithms from the operations research field while being quite fast in execution. Among the modifications that we applied to the classic PPO algorithm, communication was by far the most impactful. It significantly increased the arrival rate without compromising scalability. One particular limitation of our solution is that we train the agents in relatively small environments. Consequently, their performance may degrade as the environment scales up.



==> Flatland Competition NeurIPS 2020/teams/marmot.tex <==

\subsection{TrainfficLight: Decentralized RL for MAPF}
\label{sec:rl4}

Team \textit{MARMot-Lab-NUS}: Guillaume Sartoretti, Zhiyao Luo, Mehul Damani; 4th place RL.



\subsubsection{Method}

Our solution builds upon the multi-agent decentralized RL framework for MAPF in grid environments proposed in our previous work, PRIMAL~\cite{sartoretti2019primal}. Taking inspiration from PRIMAL, we construct a rich feature based observation for agents and use a shallow fully connected neural network architecture. We use the popular A3C learning algorithm for training~\cite{mnih2016asynchronous}. We also draw  inspiration from the use of traffic lights, which are effective in managing traffic at bottlenecks such as junctions and crossings. Despite the traffic-light-like mechanism we propose, our solution can still be implemented in a fully decentralized manner, by relying on local communication between nearby agents only.

\paragraph{State Masking}
\label{section:state_masking}

We classified the rail grid cells as described in \sectionref{sec:masking}.
Since the majority of cells in Flatland are non-decision cells and in these cells, we hard code a \texttt{MOVE\_FORWARD} action or a \texttt{STOP} action, which is determined solely by the occupancy of the single reachable neighbouring cell to ensure safety.
Correspondingly, we remove the state-action pairs of non-decision cells from training.
An obvious advantage of the state classification is that we drastically reduce the number of samples agents needed to learn in an episode.


\paragraph{Observation}

According to our state masking, decisions are only made at stopping points, i.e., a state before agents finalize their headings on a junction. The observation of an agent is tree-shaped but with a relatively shallow depth (only immediate information about the most immediate junction). Specifically, it contains a series of handcrafted and hand-selected features on the future junction (i.e., turn left, go forward and turn right). Each choices consists of 9 scalar values, including 1) whether current heading has solution to the goal 2) optimal path length to its goal, 3) number of agents blocking with in the next junction, 4) total number of agents blocking along the optimal path, 5) number of agents crashed along the optimal path, 6) total number of agents blocking on junctions along the optimal path, 7) number of agents queuing within the next junction, 8) distance to the next junction and 9) whether the closest stopping point is occupied. In total, each agent's observation is a $3 \times 9$ vector of these features, ultimately represented as a $1 \times 27$ vector.


\paragraph{Clusters}

In our solution, the real bottlenecks are not the low-level individual junction cells or switches where agents have multiple possible decisions, but are the closely connected clusters of these cells which need to be navigated effectively.
We formally define clusters as a collection of connected grid cells where each cell has at least three possible transitions (see \figureref{fig:cell_types} in \appendixref{app:cell_types}).
Since they usually consist of multiple decision cells, clusters also negatively affect tree observations by occupying a significant depth of the tree.
This makes the observation highly localized which affects the ability of agents to do long-term planning.


\paragraph{Traffic Lights}

In order to effectively resolve the bottleneck created by clusters, we propose a smart traffic light inspired mechanism that controls entry into these clusters by only allowing a single agent to occupy the cluster at a time. 
When an agent is currently occupying the cluster, the traffic light signal is red for all entry cells into the cluster. 
When there is no agent occupying the cluster, then the traffic light signal switches to green for the entry cells into the cluster which currently have an agent waiting. 
Although the implementation of this mechanism is handcrafted in our work, we believe that it would be easy to train a RL-based controller for the traffic light policy, which could make the system even more robust. This will be investigated in future works.

\paragraph{Departure Initialization}

We use two simple rules for agent initialization. 
First, we set a soft upper bound for the number of agents in the system which is a function of the grid size. 
Second, we initialize agents having the same start and end locations one after the other.
These agents generally tend to follow the same trajectory in a line and as a result, the chances of conflict between them are minimal. 

\subsubsection{Results}

Our solution\footnote{\url{https://github.com/marmotlab/flatland-challenge-neurips-2020}} achieved a score of 127.9 and was able to plan successfully for 67\% of the agents. 
The most effective component of the solution was the introduction of traffic lights, which helped prevent deadlocks and conflicts in clusters. 
Our solution, being reactive, was also relatively unaffected by malfunctions. 
We also found that departure initialization using the heuristics described above has a considerable impact on performance.


==> Flatland Competition NeurIPS 2020/teams/netcetera.tex <==
\subsection{RL with Centralized Priority Assignment}
\label{sec:rl2}

Team \textit{Netcetera}: Evgenija Spirovska, Oliver Tanevski, Aleksandar Nikov, Ramon Grunder, David Galevski, Jakov Mitrovski; 2nd place RL.

% Evgenija Spirovska, Netcetera, stevanoska.evgenija@gmail.com\\
% Oliver Tanevski, Netcetera, oliver.tanevski23@gmail.com\\
% Aleksandar Nikov, Netcetera, aleksandar.nikov@netcetera.com\\
% Ramon Grunder, Netcetera, ramon.grunder@netcetera.com\\
% David Galevski, Netcetera, david.galevski@gmail.com\\
% Jakov Mitrovski,Netcetera,jakovvmitrovski@yahoo.com	


\subsubsection{Method}
We designed an RL solution, where at each timestep each train generates an experience. We use centralized training of an Ape-X model as described in \cite{horgan2018distributed}. In the following subsections a detailed explanation for all parts of the solution is presented.

\paragraph{Representation of the Environment}
In order to optimize the calculations, we represent the environment as a graph, where each vertex represents a switch and possible arrival directions to the switch. More formally, a vertex is represented as a state-direction pair $(s,d)$. A directed edge between two vertices in the graph $(s_{1},d_{1})$ and $(s_{2},d_{2})$ exists if there is a directed path in the environment from $s1$ to $s2$, such that the directions of the train on switches match $d_{1}$ and $d_{2}$ correspondingly. A representation of a simple environment is given in \figureref{fig:graph} in \appendixref{app:graph}.

\paragraph{Representation of the State}
The state of the agent should describe its immediate surroundings well, so it can make an intelligent and informed choice for the next action. The best choice of features was obtained experimentally. Our best state representation uses a tree observation of depth 1 which includes features about the shortest path, the status and the priority of the agent and conflict information (for example: deadlock, deadlock in the next whole segment until the next usable switch). During the course of the competition we experimented with many other features, like statistical information about the path and the environment, time tick info (the number of elapsed timestamps since the beginning of the episode), info about following switches and other agents. These features proved to only create noise in the model and reduced its performance.

\paragraph{Priority}
Our model's most important feature, which led to significant improvement in its performance, was priority. The concept of priority is used for solving conflicts between agents, which happen on a regular basis during simulation. We build an undirected conflict graph, where each vertex represents an agent and the edges in the graph represent the conflicts between agents. Assigning priority to the agents is a graph coloring problem, where two neighboring vertices cannot have the same level of priority at the same time. 

We have tried several heuristics for choosing the agents that have priority. The best one was to give the highest priority to the vertex with highest degree. The logic behind this heuristic is that the agent that causes the largest number of conflicts will go first, freeing the path for most agents in the next steps.


\paragraph{Reward}
In our final reward setting, the only positive reward was reaching the target. We also included smaller and larger penalization for correcting unwanted behaviors. The biggest negative penalization was for getting into deadlock. With smaller penalization we correct not following priority, missing the shortest path, unwanted stopping, etc. 

\paragraph{Models}
Although we experimented with on-policy and off-policy models, the best results were achieved with Ape-X model. We used the RLlib library \cite{liang2018rllib} for model implementations.
We introduced the concept of curriculum learning~\citep{Bengio2009}, meaning the difficulty of the provided training environments changed over time. The idea was for the agents to learn simple behaviors first. As the training progressed, so did the complexity of the training environments, allowing the agents to learn more complex behaviors.

\subsubsection{Results}
Our solution\footnote{\url{https://github.com/netceteragroup/Flatland-Challenge}} was able to solve 228 environments, where the most complex one consisted of 181 agents and 20 cities. 88.1 \% of the agents were able to reach their target destination. Our final score was 181.5 and the reason for termination was that we reached overall the time limit of 8 hours per solution.
Our solution performs well in avoiding deadlocks. For the smaller environments, all the trains are able to reach their targets. The main disadvantage of our solution is that it is too `cautious', meaning that for really large environments more trains should be on the map simultaneously.
